Search for the Standard Model Higgs Boson Produced in Association with a $W$ Boson in the Isolated-Track Charged-Lepton Channel Using the Collider Detector at Fermilab

This dissertation presents an experimental search for the Standard Model Higgs boson produced in association to the W boson in proton antiproton collisions at a center of mass energy of 1.96 TeV and recorded with the Collider Detector at Fermilab. We improve the sensitivity of the WH search by 17% through increased signal yield by 33% by introducing a novel method to reconstruct charged lepton candidates based on an isolated track, as well as a novel method to combine triggers in order to maximize the signal yield and yet not use an OR between triggers. The observed (median expected) 95% confidence level SM Higgs upper limits on cross section times branching ratio vary between 2.39 x SM (2.73 x SM) for a Higgs mass of 100 GeV/c^2 to 31.1 x SM (31.2 x SM) for a Higgs mass of 150 GeV/c^2, while the value for a 115 GeV/c^2 Higgs boson is that of 5.08 x SM (3.79 x SM).

==> acknowledgement.tex <==
\chapter*{Acknowledgements}

\ \\This work could not have been possible without the support and help I received from many people, including, but not limited to, my supervisor, my colleagues from McGill University and the Collider Detector at Fermilab experiment, my professors from university and high school, family and friends. 

%Andreas
\ \\I am most grateful for the support I received during my MSc and PhD graduate studies at McGill University from my research supervisor, Andreas Warburton. He encouraged me to choose the topics of research that I am most enthusiastic about from the analysis topics available to me as a member of the Collider Detector at Fermilab collaboration. Therefore, I chose the low mass Standard Model Higgs boson search, the topic of this thesis. His office door was always open for me to offer updates on my research progress. His feedback was prompt, encouraging and constructive. He always answered promptly to my emails, even late at night or on weekends. The grant applications that Andreas and his faculty colleagues from CDF Canada were always succesful with NSERC, Canada's agency that funds particle physics research. As a result, I enjoyed the opportunity to travel frequently to Fermilab, the particle physics laboratory in USA where our research is performed, to the Canadian Associtation of Phycisists Congress where I presented my research results almost every year, and to other particle physics symposiums and schools. The graduate level particle physics class I took at McGill University was also taught very well by Andreas. I enjoyed the class very much and learned the basic theoretical and experimental physics that I used in my research afterwards. I was also inspired from Andreas' involvement in science outreach and contribution to the physics community in Canada. I was a graduate student representative in the Canadian Assocation of Physicists council for three years. In that period I had the opportunity to lead the local organization of a physics graduate student conference with students from across North America. Later I acted as the Canadian student contact for the same conference when it took place in Mexico. I am also very grateful for the many comments Andreas offered me in preparation for conference or regular research presentations, internal documentation and my MSc and PhD thesis. I also appreciate Andreas's insights about career paths possible in particle physics. Andreas is an excellent researcher, teacher and supervisor. I learned a lot through interaction with him. Not least, he was also a good friend to me, supporting and understanding me in difficult personal times, such as a serious car accident I had as a passenger at the beginning of my MSc studies. 

%Nils 
\ \\This work could not have been possible without the collaboration with Nils Krumnack while he was postdoctoral researcher at CDF, affiliated with Baylor University, USA. Nils taught me sound programming skills and guided my steps in implementing in code the parametrization of trigger efficiency turnon curves for three missing-transverse-energy-plus-jets triggers that I used in my analysis. It was also Nils who presented me the idea of the method to combine an unlimited number of trigger without having a logical OR between them. He also supported me while I coded the software package ABCDF for CDF that implements this idea. Nils also created code that measures the data to simulated events efficiency scale factors for isolated track events. These are key to my original contribution to  the associated production of a W boson and a Higgs boson analysis at CDF, namely the introduction of a new charged lepton category with looser reconstruction criteria, which improved the sensitivity of the analysis by 20\%. I am very greatul to Nils Krumnack for helping me get started in my own research and for teaching me a lot of coding skills. 

%Yoshikazu, Martin, Timo, Fede, Homer
\ \\I am also in debt to my fellow student colleagues from CDF: Yoshikazu Nagai (Tsukuba University, Japan), Martin Frank (Baylor University, USA), Federico Sforza (Pisa University, Italy) and Timo Aaltonen (Helsinki University, Finland). We worked together as part of the WH subgroup at CDF. I learned a lot from interaction with them, either live at Fermilab or through videoconferences and email exchanges. We exchanged advice on coding and scripting skills, on data analysis skills and presentation techniques. I interacted a lot with Yoshikazu in our effort to reproduce his WH analysis in a new data analysis framework called WHAM. Yoshikazu has answered all my questions very patiently during all this time. He also offered me his scripts, which I personalized and included in WHAM. I interacted a lot with Martin in the process of building the data ntuple tree in WHAM. I collaborated a lot with Federico while validating the background estimation method that he introduced in WHAM. I communicated a lot with Timo about the physics interpretation of the graphic results WHAM was producing. I am also very greatful to Homer Wolfe, postdoctoral researcher at CDF (Ohio State University, USA) who created the foundations and leads the effort of development for WHAM.  

%Wei-Ming, Craig, Eric, Ben, and staff
\ \\I owe a lot to the leaders of the WH subgroup at CDF (Wei-Ming Yao, BNL, USA and Craig Group, Virginia University, USA) and the conveners of the Higgs group at CDF (Eric James, Fermilab, USA, and Ben Kilminster, Fermilab, USA) who patiently followed my numerous research talks at CDF and offered me encouragement and constructive feedback and advice. I also want to help the numerous staff personnel at Fermilab who created a great atmosphere for research.  

%Paul Mercure
\ \\I also want to thank the staff at the physics departement at McGill University for all their support during my studies. Their help was essential to running things smoothly and allowing me the energy to concentrate on research. I would mention especially Paula Domingues, our secretary, who helped me most with the paperwork, Sonia Vieira, who helped with my travel reimbursement claims, Paul Mercure, who solved promptly any computing problem we might have. 

\ \\I am greateful to Teodora Dan for her help and advice in coding, especially my first classes in C++, which were to become part of the ABCDF package.

\ \\ ADD FAMILY and PROFS from PRE-HIGH SCHOOL.

